Spec$^2$R: Recovering Emergent Properties in Supervised Vision Transformers

Vision Transformers (ViTs) have achieved strong performance across computer vision tasks, but the quality of their learned representations differs drastically depending on the training paradigm. While self-supervised ViTs often demonstrate emergent properties, such as object-aligned patch representations and attention maps, supervised ViTs typically lack these properties, even when trained with strong data augmentations. Understanding the origin of this difference is important for explaining and controlling the object-level structure. To investigate it, we perform a spectral analysis of supervised and self-supervised models, and identify a key distinction: MLP layers in supervised ViTs introduce high-frequency variations into patch representations, disrupting their spatial organization. Motivated by this finding, we propose Spec$^2$R, a lightweight spectral regularization method that fine-tunes the MLP layers of pretrained supervised ViTs. Spec$^2$R recovers object-aligned patch representations and attention maps, while improving adversarial robustness and preserving competitive classification accuracy.

==> tables/app_attention_epg.tex <==

\begin{table}[t]
\centering
\caption{
\textbf{Detailed best-head Energy Pointing Game (EPG) on ImageNet-1K.}
For each transformer block, we report the attention head achieving
the highest EPG for the reference (REF) and
Spec\textsuperscript{2}R-regularized (REG) models.
Scores are expressed as percentages, and $\Delta$ denotes
the difference in percentage points.
Results are computed over 49,820 valid images.
}
\label{tab:app_epg}
\small
\setlength{\tabcolsep}{9pt}
\begin{tabular}{c cc cc r}
\toprule
\multirow{Block}
& \multicolumn{2}{c}{REF}
& \multicolumn{2}{c}{REG}
& \multirow{$\Delta$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& Head & EPG $\uparrow$ & Head & EPG $\uparrow$ & \\
\midrule
\multicolumn{6}{c}{\textbf{DeiT-III}} \\
\midrule
 1 &  8 & 61.29 &  8 & 61.29 & +0.00 \\
 2 &  9 & 65.43 &  9 & 65.43 & +0.00 \\
 3 &  5 & 69.68 &  5 & 69.68 & +0.00 \\
 4 & 12 & 69.26 & 12 & 67.69 & \textcolor{specRed}{\textbf{-1.57}} \\
 5 &  4 & 65.67 &  4 & 65.30 & \textcolor{specRed}{\textbf{-0.37}} \\
 6 &  9 & 66.33 &  9 & 67.48 & \textcolor{gainGreen}{\textbf{+1.15}} \\
 7 &  6 & 68.66 &  6 & 70.74 & \textcolor{gainGreen}{\textbf{+2.08}} \\
 8 &  3 & 73.96 &  3 & 76.13 & \textcolor{gainGreen}{\textbf{+2.17}} \\
 9 & 10 & \textbf{78.19} & 10 & 81.22 & \textcolor{gainGreen}{\textbf{+3.03}} \\
10 &  4 & 72.16 &  3 & 80.42 & \textcolor{gainGreen}{\textbf{+8.26}} \\
11 &  8 & 71.91 &  4 & 80.93 & \textcolor{gainGreen}{\textbf{+9.02}} \\
12 &  3 & 66.09 &  3 & \textbf{85.84} & \textcolor{gainGreen}{\textbf{+19.75}} \\
\midrule
\multicolumn{6}{c}{\textbf{DeiT-Distilled}} \\
\midrule
 1 & 11 & 66.42 & 11 & 66.42 & +0.00 \\
 2 &  7 & 67.40 &  7 & 67.40 & +0.00 \\
 3 &  8 & 67.06 &  8 & 67.06 & +0.00 \\
 4 &  6 & 66.81 &  6 & 66.65 & \textcolor{specRed}{\textbf{-0.16}} \\
 5 &  1 & 66.93 &  1 & 66.97 & \textcolor{gainGreen}{\textbf{+0.04}} \\
 6 &  2 & 69.02 &  2 & 69.95 & \textcolor{gainGreen}{\textbf{+0.93}} \\
 7 &  5 & 72.87 &  5 & 73.61 & \textcolor{gainGreen}{\textbf{+0.74}} \\
 8 &  5 & 73.68 &  5 & 75.21 & \textcolor{gainGreen}{\textbf{+1.53}} \\
 9 & 11 & \textbf{76.89} & 11 & 79.27 & \textcolor{gainGreen}{\textbf{+2.38}} \\
10 & 11 & 75.93 & 11 & \textbf{81.48} & \textcolor{gainGreen}{\textbf{+5.55}} \\
11 &  8 & 68.14 &  1 & 78.98 & \textcolor{gainGreen}{\textbf{+10.84}} \\
12 &  9 & 64.15 &  8 & 79.43 & \textcolor{gainGreen}{\textbf{+15.28}} \\
\midrule
\multicolumn{6}{c}{\textbf{FlexiViT}} \\
\midrule
 1 & 11 & 64.99 & 11 & 64.99 & +0.00 \\
 2 &  4 & 65.96 &  4 & 65.96 & +0.00 \\
 3 &  5 & 67.34 &  5 & 67.34 & +0.00 \\
 4 &  8 & 65.35 &  8 & 64.82 & \textcolor{specRed}{\textbf{-0.53}} \\
 5 &  3 & 63.65 &  3 & 63.02 & \textcolor{specRed}{\textbf{-0.63}} \\
 6 &  2 & 64.35 &  2 & 65.13 & \textcolor{gainGreen}{\textbf{+0.78}} \\
 7 &  8 & 67.46 &  8 & 69.03 & \textcolor{gainGreen}{\textbf{+1.57}} \\
 8 &  4 & 70.77 &  4 & 72.91 & \textcolor{gainGreen}{\textbf{+2.14}} \\
 9 & 12 & 73.04 & 12 & 75.10 & \textcolor{gainGreen}{\textbf{+2.06}} \\
10 &  5 & \textbf{73.79} &  5 & 76.57 & \textcolor{gainGreen}{\textbf{+2.78}} \\
11 &  6 & 70.85 &  5 & \textbf{77.45} & \textcolor{gainGreen}{\textbf{+6.60}} \\
12 &  7 & 65.43 &  7 & 74.78 & \textcolor{gainGreen}{\textbf{+9.35}} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/app_attention_iou.tex <==

\begin{table}[t]
\centering
\caption{
\textbf{Detailed best-head foreground IoU on PASCAL VOC 2012.}
For each transformer block, we report the head achieving the
highest foreground IoU for the reference (REF) and
Spec\textsuperscript{2}R-regularized (REG) models.
$\Delta$ denotes the improvement in percentage points.
}
\label{tab:app_voc_iou}
\small
\setlength{\tabcolsep}{9pt}
\begin{tabular}{c cc cc r}
\toprule
\multirow{Block}
& \multicolumn{2}{c}{REF}
& \multicolumn{2}{c}{REG}
& \multirow{$\Delta$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& Head & IoU $\uparrow$ & Head & IoU $\uparrow$ & \\
\midrule
\multicolumn{6}{c}{\textbf{DeiT-III}} \\
\midrule
 1 &  7 & 22.50 &  7 & 22.50 & +0.00 \\
 2 & 11 & 30.78 & 11 & 30.78 & +0.00 \\
 3 & 12 & 32.59 & 12 & 32.59 & +0.00 \\
 4 & 11 & 33.32 & 11 & 31.03 & \textcolor{specRed}{\textbf{-2.29}} \\
 5 &  4 & 34.75 &  4 & 34.41 & \textcolor{specRed}{\textbf{-0.34}} \\
 6 &  3 & 33.80 & 11 & 34.69 & \textcolor{gainGreen}{\textbf{+0.89}} \\
 7 &  3 & 36.61 &  3 & 39.27 & \textcolor{gainGreen}{\textbf{+2.66}} \\
 8 &  9 & 43.84 &  9 & \textbf{46.11} & \textcolor{gainGreen}{\textbf{+2.2}}7 \\
 9 &  5 & 36.98 &  5 & 39.66 & \textcolor{gainGreen}{\textbf{+2.68}} \\
10 &  4 & 28.83 &  8 & 34.47 & \textcolor{gainGreen}{\textbf{+5.64}} \\
11 &  8 & 23.93 &  3 & 37.07 & \textcolor{gainGreen}{\textbf{+13.14}} \\
12 & 11 & 17.04 & 11 & 40.16 & \textcolor{gainGreen}{\textbf{+23.12}} \\
\midrule
\multicolumn{6}{c}{\textbf{DeiT-Distilled}} \\
\midrule
 1 &  1 & 27.72 &  1 & 27.72 & +0.00 \\
 2 & 12 & 25.65 & 12 & 25.65 & +0.00 \\
 3 &  2 & 33.48 &  2 & 33.48 & +0.00 \\
 4 & 11 & 34.55 & 11 & 34.06 & \textcolor{specRed}{\textbf{-0.49}} \\
 5 &  3 & 35.08 &  3 & 35.00 & \textcolor{specRed}{\textbf{-0.08}} \\
 6 &  3 & \textbf{35.71} &  3 & \textbf{36.63} & \textcolor{gainGreen}{\textbf{+0.92}} \\
 7 &  4 & 31.02 &  4 & 32.48 & \textcolor{gainGreen}{\textbf{+1.46}} \\
 8 &  5 & 32.30 &  5 & 32.48 & \textcolor{gainGreen}{\textbf{+0.18}} \\
 9 & 11 & 28.05 &  4 & 27.88 & \textcolor{specRed}{\textbf{-0.17}} \\
10 &  8 & 27.03 & 12 & 27.33 & \textcolor{gainGreen}{\textbf{+0.30}} \\
11 &  8 & 18.57 &  7 & 26.61 & \textcolor{gainGreen}{\textbf{+8.04}} \\
12 &  7 & 14.65 & 12 & 33.26 & \textcolor{gainGreen}{\textbf{+18.61}} \\
\midrule
\multicolumn{6}{c}{\textbf{FlexiViT}} \\
\midrule
 1 &  2 & 23.34 &  2 & 23.34 & +0.00 \\
 2 & 12 & 28.97 & 12 & 28.97 & +0.00 \\
 3 &  8 & 34.42 &  8 & 34.42 & +0.00 \\
 4 &  2 & 30.04 &  2 & 29.71 & \textcolor{specRed}{\textbf{-0.33}} \\
 5 &  6 & 29.34 &  6 & 28.18 & \textcolor{specRed}{\textbf{-1.16}} \\
 6 &  7 & 30.95 &  6 & 32.98 & \textcolor{gainGreen}{\textbf{+2.03}} \\
 7 & 12 & 34.28 &  2 & 37.74 & \textcolor{gainGreen}{\textbf{+3.46}} \\
 8 & 11 & 41.10 & 11 & \textbf{42.93} & \textcolor{gainGreen}{\textbf{+1.83}} \\
 9 & 12 & 37.76 & 12 & 39.27 & \textcolor{gainGreen}{\textbf{+1.51}} \\
10 &  5 & 36.79 &  6 & 38.85 & \textcolor{gainGreen}{\textbf{+2.06}} \\
11 &  8 & 27.01 &  3 & 36.49 & \textcolor{gainGreen}{\textbf{+9.48}} \\
12 &  5 & 21.72 &  5 & 37.60 & \textcolor{gainGreen}{\textbf{+15.88}} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/correspondence_main.tex <==
\begin{table}[t]
    \centering
    \caption{
        \textbf{Semantic correspondence of patch representations.}
        We evaluate frozen ViT patch features using nearest-neighbor
        keypoint matching on SPair-71k and PF-PASCAL.
        We report Percentage of Correct Keypoints (PCK) at
        $(0.05, 0.10, 0.20)$.
        Best scores among original models and Spec$^2$R
        are shown in bold, the best overall scores
        are underlined.
    }
    \label{tab:semantic_correspondence}
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{lcccccc}
        \toprule
        & \multicolumn{3}{c}{\textbf{SPair-71k}}
        & \multicolumn{3}{c}{\textbf{PF-PASCAL}} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        Model
            & 0.05 $\uparrow$ & 0.10 $\uparrow$ & 0.20 $\uparrow$
            & 0.05 $\uparrow$ & 0.10 $\uparrow$ & 0.20 $\uparrow$ \\
        \midrule
        \rowcolor{dinoBlueLight}
        DINO-B/16
            & \underline{11.81} & 26.99 & 46.21
            & 28.58 & 51.41 & 69.51 \\
        \midrule
        DeiT-III-B/16
            & 7.77 & 19.60 & 37.46
            & 19.76 & 38.36 & 57.83 \\
        \rowcolor{specRedLight}
        + Spec$^2$R
            & \textbf{9.22} & \textbf{22.95} & \textbf{43.39}
            & \textbf{22.45} & \textbf{45.98} & \textbf{65.24} \\
        \midrule
        DeiT-B/16 Distilled
            & 11.31 & 27.37 & 48.16
            & 27.17 & 49.63 & 68.68 \\
        \rowcolor{specRedLight}
        + Spec$^2$R
            & \textbf{11.72} & \underline{\textbf{28.39}} & \underline{\textbf{50.06}}
            & \underline{\textbf{29.08}} & \underline{\textbf{53.77}} & \underline{\textbf{72.29}} \\
        \midrule
        FlexiViT-B/16
            & 4.26 & 11.68 & 25.16
            & 14.33 & 29.00 & 49.54 \\
        \rowcolor{specRedLight}
        + Spec$^2$R
            & \textbf{4.85} & \textbf{13.17} & \textbf{28.72}
            & \textbf{15.87} & \textbf{34.26} & \textbf{56.21} \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/temporal_tracking_main.tex <==
\begin{table}[t]
    \centering
    \caption{
        \textbf{Temporal consistency of patch representations.}
        We evaluate video object segmentation on DAVIS 2017
        using region similarity ($\mathcal{J}$), boundary accuracy
        ($\mathcal{F}$), and their mean ($\mathcal{J}\&\mathcal{F}$).
        Point tracking on TAP-Vid-DAVIS is evaluated using
        Average Jaccard (AJ), average point accuracy
        ($\delta_{\mathrm{avg}}$), and occlusion accuracy (OA).
        All metrics are reported in \% ($\uparrow$).
        Best scores among original supervised models and
        Spec$^2$R variants are shown in bold, while the
        best overall scores are underlined.
    }
    \label{tab:temporal}
    \scriptsize
    \setlength{\tabcolsep}{5.5pt}
    \begin{tabular}{lcccccc}
        \toprule
        & \multicolumn{3}{c}{\textbf{DAVIS 2017}}
        & \multicolumn{3}{c}{\textbf{TAP-Vid-DAVIS}} \\
        \cmidrule(lr){2-4}
        \cmidrule(lr){5-7}
        Model
            & $\mathcal{J}\uparrow$
            & $\mathcal{F}\uparrow$
            & $\mathcal{J}\&\mathcal{F}\uparrow$
            & AJ $\uparrow$
            & $\delta_{\mathrm{avg}}\uparrow$
            & OA $\uparrow$ \\
        \midrule
\rowcolor{dinoBlueLight}
DINO-B/16
    & \underline{59.37} & \underline{62.18} & \underline{60.77}
    & -- & -- & -- \\
\midrule
DeiT-III-B/16
    & 53.73 & 55.80 & 54.76
    & -- & -- & -- \\
\rowcolor{specRedLight}
+ Spec$^2$R
    & \textbf{55.19} & \textbf{56.73} & \textbf{55.96}
    & -- & -- & -- \\
\midrule
DeiT-B/16 Distilled
    & 56.96 & 60.03 & 58.50
    & -- & -- & -- \\
\rowcolor{specRedLight}
+ Spec$^2$R
    & \textbf{58.19} & \textbf{60.55} & \textbf{59.37}
    & -- & -- & -- \\
\midrule
FlexiViT-B/16
    & 50.66 & 53.90 & 52.28
    & -- & -- & -- \\
\rowcolor{specRedLight}
+ Spec$^2$R
    & \textbf{52.20} & \textbf{54.78} & \textbf{53.49}
    & -- & -- & -- \\
\bottomrule
    \end{tabular}
\end{table}

==> tables/token_cut_main.tex <==
\begin{table}[t]
    \centering
    \caption{
        \textbf{Unsupervised object discovery from patch representations.}
        We evaluate frozen ViT patch features using TokenCut
        on PASCAL VOC 2007, VOC 2012, and COCO20K.
        We report Correct Localization (CorLoc) at IoU threshold 0.5.
        Best scores among original models and Spec$^2$R
        are shown in bold, the best overall scores
        are underlined.
    }
    \label{tab:object_discovery}
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{lccc}
        \toprule
        Model
            & VOC07 $\uparrow$
            & VOC12 $\uparrow$
            & COCO20K $\uparrow$ \\
        \midrule
        \rowcolor{dinoBlueLight}
        DINO-B/16
            & \underline{57.37}
            & \underline{62.54}
            & \underline{48.20} \\
        \midrule
        DeiT-III-B/16
            & 21.21 & 22.54 & 14.98 \\
        \rowcolor{specRedLight}
        + Spec$^2$R
            & \textbf{35.66}
            & \textbf{40.35}
            & \textbf{28.63} \\
        \midrule
        DeiT-B/16 Distilled
            & 52.62 & 56.22 & 45.72 \\
        \rowcolor{specRedLight}
        + Spec$^2$R
            & \textbf{54.44}
            & \textbf{59.35}
            & \textbf{46.12} \\
        \midrule
        FlexiViT-B/16
            & 11.14 & 14.79 & 9.28 \\
        \rowcolor{specRedLight}
        + Spec$^2$R
            & \textbf{40.99}
            & \textbf{46.74}
            & \textbf{32.36} \\
        \bottomrule
    \end{tabular}
\end{table}
